Everything is a Race and Nakamoto Always Wins

Nakamoto invented the longest chain protocol, and claimed its security by analyzing the private double-spend attack, a race between the adversary and the honest nodes to grow a longer chain. But is it the worst attack? We answer the question in the affirmative for three classes of longest chain protocols, designed for different consensus models: 1) Nakamoto's original Proof-of-Work protocol; 2) Ouroboros and SnowWhite Proof-of-Stake protocols; 3) Chia Proof-of-Space protocol. As a consequence, exact characterization of the maximum tolerable adversary power is obtained for each protocol as a function of the average block time normalized by the network delay. The security analysis of these protocols is performed in a unified manner by a novel method of reducing all attacks to a race between the adversary and the honest nodes.

==> Chia_Model.tex <==

\begin{enumerate}
    
     \item $\tau_i$ = generation time of the $i$-th honest block; $\tau_0 = 0$ is the mining time of the genesis block, $\tau_{i+1} - \tau_i$ is exponentially distributed with mean $1/\lambda_h$, i.i.d. across all $i$'s. 
    Suppose an honest block $B$ is generated at time $\tau_j$.  If $\tau_j - \tau_{j-1} > \Delta$, then we call $B$ is a {\it non-tailgater} (otherwise, $B$ is a {\it tailgater}). If $\tau_j - \tau_{j-1} > \Delta$ and $\tau_{j+1} - \tau_j > \Delta$, then we call $B$ is a {\it loner}. Note that non-tailgaters have different depths and a loner is the only honest block at its depth.
    %\item $\omega_i$ = arrival time of the $i$-th non-tailgater; $\omega_0 = 0$ is the arrival time of the genesis block. Note that non-tailgaters have different depths.
    %\item $\theta_i$ = arrival time of the $i$-th loner; $\theta_0 = 0$ is the arrival time of the genesis block. Note that a loner is the only honest block at its depth.
    \item $\B(s,t)$, $s<t$ is a fictitious random tree process consisting of only the honest blocks that arrive within the time period $[s,t]$ and constructed in the following way: Let the $i$-th honest block $h_i$ be the last honest block that arrived before time $s$ (i.e., $\tau_i \leq s < \tau_{i+1}$). This block will be denoted as the ``origin'' block of the process $\B(s,t)$. Each new honest block $h_m$ that arrives within the interval $[s,t]$ will choose the last honest block before time $\tau_m - \Delta$ as its parent. If $\tau_m - \Delta \leq \tau_i$, then $h_m$ will be discarded. Let $H(s,t)$ denote the depth reached by $\B(s,t)$. Note that the depth of the origin block is $0$. Observe that when $\Delta=0$, $H(s,t)$ will be exactly equal to the number of honest blocks that arrive within the interval $[s,t]$. Then for $\Delta = 0$, we can write $H(s,t) = A_h(t) - A_h(s)$, where $A_h(t)$ is the number of honest blocks generated from time $0$ to $t$ and it increases by $1$ at each time $\tau_i$. $A_h(\cdot)$ is a Poisson process of rate $\lambda_h$.
    
    \item $L^{(p)}(t)$ is the length of $\C^{(p)}(t)$ for each $1 \leq p \leq n$. $L^{(p)}(0) = 0$. Note that since every non-tailgater appears at different depth in the block tree, it follows Proposition \ref{prop:delay} that for all $t > s+\Delta$ 
    \begin{equation} L^{(p)}(t)- L^{(p)}(s) \ge H(s,t-\Delta).
    \label{eq:lc_growth_chia}
    \end{equation}
    
    \item Notice that when $\Delta=0$, $\T^{(p)}(t)=\T^{(q)}(t)$ for all miners $1 \leq p,q \leq n$. Then $\C^{(p)}(t)=\C^{(q)}(t)=\C(t)$ for all miners $1 \leq p,q \leq n$. Consequently, when $\Delta=0$, there exists a single public longest chain $\C(t)$ at any time $t$. This $\C(t)$ is updated in two possible ways: 1) An honest block is appended to $\C(t)$ if an arrival from the honest process occurs at time $t$. 2) The adversary can replace $\C(t^-)$ by another chain $\C(t)$ from $\T(t)$ which is equal or longer in length than $\C(t^-)$. Let $L(t)$ be the length of $\C(t)$. $L(0) = 0$. Note that since the chain $\C(t)$ increments by $1$ for every honest block generation when $\Delta = 0$, (\ref{eq:lc_growth_chia}) becomes for all $i$ and for all $t > \tau_i$,  
    \begin{equation} L(t)- L(\tau_i) \ge H(\tau_i,t) = A_h(t) - A_h(\tau_i).
    \label{eq:lc}
    \end{equation}
    
    %Actually, the growth rate of $\C(t)$ should be $1/(1+\Delta)$ rather than $g$ since not every tailgater is ‘‘wasted'' (e.g., if a non-tailgater $B_1$ is mined at time $t$, block $B_2$ is mined at time $t + \frac{2\Delta}{3}$, and block $B_3$ is mined at time $t + \frac{4\Delta}{3}$, then both $B_2$ and $B_3$ are tailgater but $B_3$ will appear at a different depth from $B_1$). And we always have $1/(1+\Delta) > g$, thus counting the number of non-tailgaters do not provide the tightest result for chain growth.
    \item $\tt_i = \{\tt_i(s) : s \ge 0\}$ is the random tree process generated by the adversary starting from the $i$-th honest block. $\tt_i(0)$ consists of the $i$-th honest block and $\tt_i(s)$ consists of all adversarial blocks grown on the $i$-th honest block from time $\tau_i$ to $\tau_i + s$. Note that the $\tt_i$'s are i.i.d. copies of the adversarial tree $\T^a$. Note that the overall tree $\T(t)$ is the composition of the adversarial trees $\T_0(t), \T_1(t-\tau_1), \ldots \T_i(t - \tau_i)$ where the $i$-th honest block is the last honest block that was generated before time $t$. How these trees are composed to form $\T(t)$ depends on the adversarial action on when to release the private chains.
    \item $D_i(s)$ is the depth of the adversarial tree $\tt_i(s)$. 

\end{enumerate}

%The longest chain protocol means that the honest nodes always %%propose on the tip of the current public longest chain $\C(t)$ %%(at rate $\lambda_h$, proportional to their stake). The %%adversary can propose on any block (at rate $\lambda_a$, again %%proportional to its stake.) 
 Also the adversary has the ability to have a message delivered to honest nodes at different times (but all within $\Delta$ time). 

Proving the security (liveness and persistence) of the protocol boils down to  providing a guarantee that the chain $\C(t)$ converges as $t \rightarrow \infty$ regardless of the adversary's strategy. We study this in the next section, here first defining the following events which will be helpful for demonstrating the convergence of the longest chain:
\begin{equation}
    E_{ij} = \mbox{event that $D_i(t - \tau^h_i) < H(\tau^h_i, t-\Delta)$ for all $t > \tau^h_j+\Delta$}.
\end{equation}
and 
\begin{equation}
F_j = \bigcap_{i = 0}^{j-1} E_{ij}.
\end{equation}

$U_j$ is the event that the $j$-th honest block is a loner:
\begin{equation}
U_j = \{\tau_j - \tau_{j-1} > \Delta, \tau_{j+1} - \tau_j > \Delta\}
\end{equation}
When $\Delta=0$, every block is a loner. 

Finally, we define the adversary-proof convergence event: 
\begin{equation}
\hat{F}_j = F_j \cap U_j    
\end{equation}
Note that $\hat{F}_j$ reduces to $F_j$ when $\Delta=0$. Hence, when $\Delta=0$, the adversary-proof convergence event will be denoted by $F_j$.

These events can be interpreted as about a fictitious system where there is a growing chain consisting of only honest blocks. The event $E_{ij}$ is the event that the adversarial tree rooted at the $i$-th honest block does not catch up with the honest chain any time after the generation of the $j$-th honest block. Such a tree can be interpreted as providing resource for a possible attack at the honest chain. If $E_{ij}$ occurs, then there is not enough resource for the $i$-th tree to attack after the $j$-th block. If $F_j$ occurs, there is not enough resource for {\em any} of the previous trees to attack the honest chain. 

Even though the events are about a fictitious system with a purely honest chain and the longest chain in the actual system may consist of a mixture of adversarial and honest blocks, intuitively the actual chain can only grow faster than the fictitious honest chain.

==> Nakamoto_Model.tex <==
 We also assume that there are an infinite number of honest miners, each of which has an infinitesimal block generation rate. This assumption, which we denote as the `infinitesimal miner assumption', enables us to assert that a miner can mine at most one block within any given closed interval. 

\begin{enumerate} 
\item $\tau^h_i$ and $\tau^a_i$ are defined as the generation times of the $i$-th honest and adversary blocks respectively. $\tau_0 = 0$ is the generation time of the genesis block. $T^h_{i+1} := \tau^h_{i+1} - \tau^h_i$ and $T^a_{i+1} := \tau^a_{i+1} - \tau^a_i$ are exponentially distributed with means $1/\lambda_h$ and $1/\lambda_a$ respectively, i.i.d. across all $i$'s.

\item Suppose an honest block $h_j$ is generated at time $\tau^h_j$. If $\tau^h_j - \tau^h_{j-1} > \Delta$, then we call $h_j$ a {\it non-tailgater} (otherwise, it is a {\it tailgater}). If $\tau^h_j - \tau^h_{j-1} > \Delta$ and $\tau^h_{j+1} - \tau^h_j > \Delta$, then we call $h_j$ a {\it loner}. Note that non-tailgaters have different depths and a loner is the only honest block at its depth.


 
\end{enumerate}

When $\Delta=0$, the longest chain protocol implies that the honest miners always mine on the tip of the current public longest chain $\C(t)$ with rate $\lambda_h$. However, the adversary can still change where the honest nodes act by broadcasting a chain of equal or longer length than $\C(t^-)$ at time $t$ using the blocks in $\T(t)$. Since the adversary can change where the honest blocks can be mined even with an equal length new chain, the adversary is given the ability to choose where the honest nodes mine when there are more than one public longest chain.

We next define several basic random variables and processes which are constituents of the processes $\T(\cdot)$ and $\C(\cdot)$. We then use them to define the notion of the adversary-proof convergence event in the context of the longest chain protocol, and show that, once this event occurs, convergence of the common prefix for the longest chains will occur regardless of the adversarial action. 

Define $\tt_i = \{\tt_i(s) : s \ge 0\}$ as the random tree process generated by the adversary starting from the $i$-th honest block. $\tt_i(0)$ consists of the $i$-th honest block and $\tt_i(s)$ consists of all the adversary blocks grown on the $i$-th honest block from time $\tau^h_i$ to $\tau^h_i + s$. Let $D_i(s)$ denote the depth of the adversarial tree $\tt_i(s)$. Observe that the overall tree $\T(t)$ is composed of the adversarial trees $\T_0(t-\tau^h_0), \T_1(t-\tau^h_1), \ldots \T_i(t-\tau^h_i)$ where the $i$-th honest block is the last honest block that was generated before time $t$. How these trees are composed to form $\T(t)$ depends on the adversarial action on when to release its private chains.

We next define $\B(s,t)$, $s<t$, as a fictitious random tree process consisting of only the honest blocks that arrive within the time period $[s,t]$ and constructed in the following way: Let the $i$-th honest block $h_i$ be the last honest block that arrived before time $s$ (i.e., $\tau^h_i \leq s < \tau^h_{i+1}$). This block will be denoted as the ``origin'' block of the process $\B(s,t)$. Each new honest block $h_m$ that arrives within the interval $[s,t]$ will choose the last honest block before time $\tau^h_m - \Delta$ as its parent. Moreover, each block will `appear' in the tree $\B(s,t)$ $\Delta$ time after it arrives. If $\tau^h_m - \Delta \leq \tau^h_i$, then $h_m$ will be placed at the same depth as $h_i$. Let $H(s,t)$ denote the depth reached by $\B(s,t)$. Note that the depth of the origin block is $0$. Also observe that when $\Delta=0$, $H(s,t)$ will be exactly equal to the number of honest blocks that arrive within the interval $[s,t]$.

Finally, let us define the following events which will be helpful for demonstrating the convergence of the longest chain in the subsequent sections:

$E_{ij}$ is the event that $D_i(t - \tau^h_i) < H(\tau^h_i, t-\Delta)$ for all $t > \tau^h_j+\Delta$.
\begin{equation}
    F_j = \bigcap_{0 \leq i < j} E_{ij},
\end{equation}

$U_j$ is the event that the $j$-th honest block is a loner:
\begin{equation}
U_j = \{\tau_j - \tau_{j-1} > \Delta, \tau_{j+1} - \tau_j > \Delta\}
\end{equation}
When $\Delta=0$, every block is a loner. 

Finally, we define the adversary-proof convergence event: 
\begin{equation}
\hat{F}_j = F_j \cap U_j    
\end{equation}
Note that $\hat{F}_j$ reduces to $F_j$ when $\Delta=0$. Hence, when $\Delta=0$, the adversary-proof convergence event will be denoted by $F_j$.

These events can be interpreted as about a fictitious system where there is a growing chain consisting of only honest blocks. The event $E_{ij}$ is the event that the adversarial tree rooted at the $i$-th honest block does not catch up with that honest chain any time after the generation of the $j$-th honest block. Such a tree can be interpreted as providing resource for a possible attack at the honest chain. If $E_{ij}$ occurs, then there is not enough resource for the $i$-th tree to attack after the $j$-th block. If $F_j$ occurs, there is not enough resource for {\em any} of the previous trees to attack the honest chain. 

Even though the events are about a fictitious system with a purely honest chain and the longest chain in the actual system may consist of a mixture of adversarial and honest blocks, intuitively the actual chain can only grow faster than the fictitious honest chain, and so we have the following key lemmas \ref{lem:regen} and \ref{lem:loner}. These lemmas justify us giving the name {\em adversary-proof convergence event} to $F_j$.

For the proof of these lemmas, it is crucial to show that $H(s,t)$ gives a conservative bound on the growth of the chains $\C^{(p)}$ from time $s$ to $t$ for any $s < t - \Delta$. For this purpose, before moving onto the lemmas \ref{lem:regen} and \ref{lem:loner}, we prove the following proposition:

\begin{proposition}
\label{prop:delay}
For any given $s$, $t$ such that $s < t - \Delta$;
$$H(s,t-\Delta) \leq L^{(p)}(t)-L^{(p)}(s)$$
for any honest miner $p$.
\end{proposition}

\begin{proof}
Assume that the increase in $L^{(p)}$ within the interval $[s,t]$ is solely due to the arrival of honest blocks in the interval $[s-\Delta,t]$. Then, we first show that delaying every block that arrives within this interval by $\Delta$ minimizes the increase in $L^{(p)}$ for any time $t>s$. To prove this, first observe that minimizing the increase in $L^{(p)}$ is equivalent to maximizing the time it takes for $\C^{(p)}$ to reach any further depth $d$. Now, let $h_i$ be the block at the tip of $\C^{(p)}$ when it reaches depth $d$, and, assume that it took $\delta_i \leq \Delta$ time for $p$ to learn about $h_i$ after it was mined. Then, $\C^{(p)}$ reaches depth $d$ at time $\tau^h_i+\delta_i$. However, if the message for $h_i$ was delayed for $\delta'_i>\delta_i$ time, then, either $\C^{(p)}$ would have reached depth $d$ at time $\tau^h_i+\delta'_i \geq \tau^h_i+\delta_i$ with block $h_i$ at its tip or another block $h_j$, with index $j \neq i$ would have brought $\C^{(p)}$ to depth $d$ at some time $t$, $\tau^h_i+\delta'_i > t > \tau^h_i+\delta_i$. Hence, delaying the transmission of $h_i$ increases the time it takes for $\C^{(p)}$ to reach depth $d$. This implies that $h_i$ should be delayed as long as possible, which is $\Delta$. Since this argument also applies to any other block $h_j$ that might also bring $\C^{(p)}$ to depth $d$ when $h_i$ is delayed, every block should be delayed by $\Delta$ to maximize the time for $\C^{(p)}$ to reach any depth $d$. This, in turn, minimizes the increase in $L^{(p)}$ by any time $t>s$. 

We next observe that when every honest block is delayed by $\Delta$, the increase in $L^{(p)}$ that only receives honest blocks within interval $[s,t]$ is lower bounded by $H(s,t-\Delta)$. Now, the adversary blocks arriving within this interval can only contribute to the increase in $L^{(p)}$ due to the longest chain protocol. We also know from the above paragraph that delaying every honest block by $\Delta$ minimizes $L^{(p)}(t)-L^{(p)}(s)$ when only honest blocks come to $\C^{(p)}$. Hence, we can conclude that;
$$H(s,t-\Delta) \leq L^{(p)}(t)-L^{(p)}(s)$$
for any honest miner $p$.

\end{proof}


==> Security_Analysis_Chia_0.tex <==

{\bf \noindent Occurrence of adversary-proof convergence }
If the growth rate of the adversarial tree is greater than $\lambda_h$, then the adversary can always attack the honest chain by growing a side chain at a rate faster than the honest chain's growth rate and replace it at will. (\ref{eq-Ofer2}) immediately shows that if  $\lambda_a  > \lambda_h/e$, i.e. when the adversarial fraction $\beta > 1/(1+e)$, the growth rate of the adversarial tree is at least $1$, and hence the private attack is successful. This is what \cite{fan2018scalable} showed. The question we want to answer is what happens when $\beta < 1/(1+e)$? Will another attack work? 
%We show below that 
We show below that in this regime,  the adversary-proof convergence event $F^0_j$ has a non-zero probability of occurrence, and this implies that no attack works. 



\begin{lemma}
\label{lem:infinite_E}
If $\lambda_a < \lambda_h/e$, i.e. $\beta < 1/(1+e)$, then there exists a strictly positive constant $p> 0 $ such that $P(F^0_j) \ge p$ for all $j$. Also, with probability $1$, the event $F^0_j$ occurs for infinitely many $j$'s.
\end{lemma}

The proof of this result can be found in \S\ref{app:proof_0_delay}.


{\bf \noindent Waiting time for convergence}
In the previous section, we established the fact that the event $F^0_j$ has  $P(F^0_j) > p > 0$ for all $j$. This implies that the event $F^0_j$ occurs infinitely often. But how long do we need to wait for such an event to occur? We answer this question in the present section.

More specifically, we would like to get a bound on the probability that in a time interval $[s,s+t]$, there are no adversary-proof convergence events, i.e.  a bound on:
$$q[s,s+t] :=P(\bigcap_{j: \tau^h_j \in [s,s+t]} F^0_j^c).$$


\begin{lemma}
\label{lem:time-zero-delay}
If $\lambda_a< \lambda_h/e$, i.e. $\beta < 1/(1+e)$ then there exist constants $a_2,A_2$ so that, for any $s,t\geq 0$, 
\begin{equation}
\label{eq-satofer1}
q[s,s+t] \;\; \leq \;\; A_2\exp(-a_2\sqrt{t}).
\end{equation}
%for some constants $a_2,A_2 > 0$.
%and a polynomial $A_2(t)$.
\end{lemma}
\noindent The bound in \eqref{eq-satofer1} is not optimal, see Remark \ref{rem-1} below.
\begin{proof}
Define $R_j = \tau^h_{j+1}- \tau^h_j$, and let 
\begin{equation}
    B_{ik} = \mbox{event that $D_i(\sum_{m = i}^{k-1} R_m) \; \ge \;  (k - i-1)
    $}.
\end{equation}
(Notation as in \eqref{eq-Bik}.)
Note that from Lemma~\ref{theo-tail} we have 
\begin{eqnarray}
\label{eq-PBik}
  P(B_{ik})
    &\le & P\left (B_{ik}|\sum_{m = i}^{k-1} R_m < (k-i-1) \frac{\lambda_h+\lambda_a e}{2\lambda_a e}\frac{1}{\lambda_h} \right)\nonumber\\
    &+& P\left(\sum_{m = i}^{k-1} R_m \geq (k-i-1) \frac{\lambda_h+\lambda_a e}{2\lambda_a e}\frac{1}{\lambda_h} \right) \nonumber\\
    & \le &  \left( \frac{\lambda_h +e\lambda_a}{2\lambda_h} \right)^{k-i-1} + A_1 e^{-\alpha_1 (k-i-1)}
\end{eqnarray}
for some positive  constants $A_1, \alpha_1$ independent of $k,i$. The first term in the last inequality follows from (\ref{eq:Ofertheo}), and the second term follows from the fact that $(\lambda_h+\lambda_a e)/(2\lambda_a e) > 1$ and the $R_i$'s are iid exponential random variables  of mean $1/\lambda_h$. 
\iffalse
\begin{eqnarray*}
P(B_{ik}|\tau^h_k-\tau^h_i=t) &=& P(D_i(\tau^h_k-\tau^h_i)\geq k-i-1|\tau^h_k-\tau^h_i)\\
&\leq& e^{-(k-i-1)+e\lambda_a t}\;,
\end{eqnarray*}
and taking expectation over $t=\tau^h_k-\tau^h_i$ we get
\begin{eqnarray*}
P(B_{ik}) &\leq & e^{-(k-i-1)}\prod_{j=i}^{k-1} E[e^{e\lambda_a R_j}]\\
    &=&e^{-(k-i-1)}\prod_{j=i}^{k-1}\Big(\frac{\lambda_h}{\lambda_h-e\lambda_a}\Big)^{k-i} \\
    &=& e^{1-(k-i) }
\end{eqnarray*}
{\bf Xuechao: can you fill this in?}
\fi
Then 
\begin{equation}
    F^0_j^c = \bigcup_{(i,k): i < j, k >j} B_{ik}.
\end{equation}
Divide $[s,s+t]$ into $\sqrt{t}$ sub-intervals of length $\sqrt{t}$, so that the $r$ th sub-interval is:
$$\J_r : = [s+  (r-1) \sqrt{t}, s+ r\sqrt{t}].$$

Now look at the first, fourth, seventh, etc sub-intervals, i.e. all the $r = 1 \mod 3$ sub-intervals. Introduce the event that in the $\ell$-th $1 \mod 3$th sub-interval,
an adversarial tree that is rooted at a honest block arriving in that sub-interval or in the previous ($0 \mod 3$) sub-interval catches up with a honest block in that sub-interval or in the next ($2 \mod 3$) sub-interval. 
Formally,
$$C_{\ell}=\bigcap_{j: \tau^h_j \in \J_{3\ell+1}}
\bigcup_{(i,k): \tau^h_j - \sqrt{t} < \tau^h_i < \tau^h_j, \tau^h_j < \tau^h_k < \tau^h_j +\sqrt{t} } B_{ik}.$$
Note that for distinct $\ell$, the events $C_\ell$'s  are independent. Also, we have
\begin{equation}
    \label{eq-qq2}
    P(C_{\ell})\leq P(\mbox{no arrival in $\J_{3\ell+1}$}) + 1-p < 1
    \end{equation}
for large enough $t$. 

Introduce the atypical events:
\begin{eqnarray}
    B &=& \bigcup_{(i,k): \tau^h_i \in [s,s+t] \mbox{~or~} \tau^h_k \in [s,s+t], i <k, \tau^h_k - \tau^h_i >  \sqrt{t}} B_{ik} \;, \text{ and }\\
    \tilde{B} &=& 
    \bigcup_{(i,k):\tau^h_i<s,s+t<\tau^h_k} B_{ik}\;.
\end{eqnarray}
The events $B$ and $\tilde{B}$ are the events  that an adversarial tree catches up with an honest block far ahead. 
Consider also the events
\begin{eqnarray}
D_1&=&\{\# \{i: \tau^h_i\in (s-\sqrt{t},s+t+\sqrt{t})\} >2\lambda_h t\} \label{D1}\\
D_2&=& \{ \exists i,k: \tau^h_i  \in (s,s+t), (k-i)<\sqrt{t}/2\lambda_h,
\tau^h_k-\tau^h_i>\sqrt{t}\} \label{D2}\\
D_3&=& \{ \exists i,k: \tau^h_k \in (s,s+t), (k-i)<\sqrt{t}/2\lambda_h,
\tau^h_k-\tau^h_i>\sqrt{t}\} \label{D3}
\end{eqnarray}
In words, $D_1$ is the event of atypically many honest arrivals in $(s-\sqrt{t},s+t+\sqrt{t})$ while $D_2$ and $D_3$ are the events that there exists an interval 
of length $\sqrt{t}$ with at least one endpoint 
inside $(s,s+t)$ with atypically small number of 
arrivals. Since the number of honest arrivals in $(s,s+t)$ is Poisson with parameter $\lambda_h t$, we have from the memoryless property of the Poisson process that  $P(D_1)\leq e^{-c_0t}$ for some constant $c_0=c_0(\lambda_a,\lambda_h)>0$.  On the other hand, using the memoryless property and a union bound, and decreasing $c_0$ if needed, we have
that $P(D_2)\leq e^{-c_0 \sqrt{t}}$. Similarly, using time reversal, $P(D_3)\leq e^{-c_0\sqrt{t}}$. Therefore,
again using the memoryless property of the Poisson process,
\begin{eqnarray}
P(B)&\leq & P(D_1\cup D_2\cup D_3)+ P(B\cap D_1^c\cap D_2^c\cap D_3^c)\nonumber\\
&\leq & e^{-c_0 t} + 2e^{-c_0\sqrt{t}}+\sum_{i=1}^{2\lambda_h t} \sum_{k: k-i>\sqrt{t}/2\lambda_h}
P(B_{ik})\leq c_1e^{-c_2\sqrt{t}},
\label{eq-thursday8}
\end{eqnarray}
where $c_1,c_2>0$ are constants that may depend on
$\lambda_a,\lambda_h$ and the last inequality is due to \eqref{eq-PBik}.
%By using Lemma \ref{theo-tail} and  a union bound we have that $P(B) \leq c_1 e^{-c_2 \sqrt{t}}$ for some constants $c_1,c_2>0$.
%polynomial $a_2(t)$ and constant $c_2$. 
%%    Indeed, we would have had equality in \eqref{eq-qq} if the union were over all $s$.
We next claim that there exists a constant $\alpha>0$ so that,
for all $t$ large,
\begin{equation}
    \label{eq-thursday1}
    P(\tilde B)\leq e^{- \alpha t}.
    \end{equation}
    Indeed, we have that
    \begin{eqnarray}
    P(\tilde B)&=&
    \sum_{i<k} \int_0^s P(\tau^h_i\in d\theta)
    P(B_{ik}, \tau^h_k-\tau^h_i>s+t-\theta)\nonumber \\
    &\leq & \sum_i \int_0^s 
    P(\tau^h_i\in d\theta) \sum_{k:k>i} P(B_{i,k})^{1/2}
    P(\tau^h_k-\tau^h_i>s+t-\theta)^{1/2}.
    \label{eq-thursday2}
    \end{eqnarray}
    By \eqref{eq-PBik}, there exists $c_3>0$ so that
    \begin{equation}
        \label{eq-thursday1bis}
    P(B_{i,k})\leq e^{-c_3(k-i-1)},
    \end{equation}
    while the tails of the
    Poisson distribution yield the existence of constants
    $c,c'>0$ so that
    \begin{equation}
        \label{eq-thursday3}
        P(\tau^h_k-\tau^h_i>s+t-\theta)=
        P(\tau^h_{k-i}>s+t-\theta)
        \leq \left\{
        \begin{array}{ll}
        1,& (k-i)>c(s+t-\theta)\\
        e^{-c'(s+t-\theta)},& (k-i)\leq c(s+t-\theta).
        \end{array}\right.
    \end{equation}
    Combining \eqref{eq-thursday1bis} with \eqref{eq-thursday3}
   yields that there exists a constant $\alpha>0$ so that
    \begin{equation}
        \label{eq-thursday4}
        \sum_{k: k>i} P(B_{i,k})^{1/2}P(\tau^h_k-\tau^h_i>s+t-\theta)^{1/2}
        \leq e^{-2\alpha(t+s-\theta)}.
    \end{equation}
    Substituting this bound in \eqref{eq-thursday2} and using that $\sum_i P(\tau^h_i\in d\theta)=d\theta$ gives
    \begin{eqnarray}
    \label{eq-thursday5}
    P(\tilde B)&\leq &
    \sum_{i} \int_0^s 
    P(\tau^h_i\in d\theta) e^{-2\alpha (t+s-\theta)}\nonumber\\
    &\leq& \int_0^s e^{-2\alpha (t+s-\theta)} d\theta
    \leq e^{-\alpha t},
    \end{eqnarray}
    for $t$ large, proving \eqref{eq-thursday1}.
    
    Continuing with the proof of the lemma, we have: 
\begin{eqnarray}
\label{eq-qqq2}q[s,s+t] &\leq& P(B)+P(\tilde B)+P(\bigcap_{\ell=0}^{\sqrt{t}/3} C_{\ell})\nonumber \\
&=& P(B)+ P(\tilde B)+(P(C_{\ell}))^{\sqrt{t}/3}\nonumber \\
&\leq& c_1 e^{-c_2\sqrt{t}}+ e^{-\alpha t} + (P(C_\ell))^{\frac{\sqrt{t}}{3}}
\end{eqnarray}
where the equality is due to independence, and in
the last inequality we used \eqref{eq-thursday8} and \eqref{eq-thursday1}. The lemma follows from
\eqref{eq-qq2}.
\end{proof}
\begin{remark}
\label{rem-1}
Iterating the proof above  (taking  longer 
blocks and using the bound of Lemma \ref{lem:time-zero-delay} to improve on $P(C_\ell)$ in \eqref{eq-qq2} by replacing $p$ with the bound from 
\eqref{eq-satofer1})
shows that \eqref{eq-satofer1} can be improved to the statement
that for any $\theta>1$ there exist constants $a_\theta,A_\theta$ so that, for any $s,t>0$,
\begin{equation}
\label{eq-satofer2}
q[s,s+t] \;\; \leq \;\; A_\theta\exp(-a_\theta t^{1/\theta}).
\end{equation}
\end{remark}

\iffalse
$\B(s,t)$, $s<t$ is a fictitious random tree process consisting of only the honest blocks that arrive within the time period $[s,t]$ and constructed in the following way: Let the $i$-th honest block $h_i$ be the last honest block that arrived before time $s$ (i.e., $\tau^h_i \leq s < \tau^h_{i+1}$). This block will be denoted as the ``origin'' block of the process $\B(s,t)$. Each new honest block $h_m$ that arrives within the interval $[s,t]$ will choose the last honest block before time $\tau^h_m - \Delta$ as its parent. If $\tau^h_m - \Delta \leq \tau^h_i$, then $h_m$ will be discarded. Let $H(s,t)$ denote the depth reached by $\B(s,t)$. Note that the depth of the origin block is $0$. Observe that when $\Delta=0$, $H(s,t)$ will be exactly equal to the number of honest blocks that arrive within the interval $[s,t]$. Then for $\Delta = 0$, we can write $H(s,t) = A_h(t) - A_h(s)$, where $A_h(t)$ is the number of honest blocks generated from time $0$ to $t$ and it increases by $1$ at each time $\tau^h_i$. $A_h(\cdot)$ is a Poisson process of rate $\lambda_h$.
\fi


==> Security_Analysis_Delta_0.tex <==
\begin{comment}

{\bf \noindent Adversary-proof convergence }
We first define several basic random variables and processes which are constituents of the processes $\T(\cdot)$ and $\C(\cdot)$ in the Nakamoto Proof-of-Work model. We then use them to define the notion of the `adversary-proof convergence' event in the context of the longest chain protocol, and show that, once this event occurs, convergence of the common prefix for the longest chains will occur regardless of the adversarial action. 

Define $\tt_i = \{\tt_i(s) : s \ge 0\}$ as the random tree process generated by the adversary starting from the $i$-th honest block. $\tt_i(0)$ consists of the $i$-th honest block and $\tt_i(s)$ consists of all the adversary blocks grown on the $i$-th honest block from time $\tau^h_i$ to $\tau^h_i + s$. Let $D_i(s)$ denote the depth of the adversarial tree $\tt_i(s)$. Observe that the overall tree $\T(t)$ is composed of the adversarial trees $\T_0(t-\tau^h_0), \T_1(t-\tau^h_1), \ldots \T_i(t-\tau^h_i)$ where the $i$-th honest block is the last honest block that was generated before time $t$. How these trees are composed to form $\T(t)$ depends on the adversarial action on when to release its private chains.

We next define $\T_h(t)$ as a fictitious random process consisting of all the honest blocks that arrived by time $t$. For any given sequence of arrival times for the honest blocks up till time $t$, $\T_h(t)$ gives an ordering for the depths of these honest blocks. In this context, define $d^h_i$ as the depth of the $i$-th honest block $h_i$ within $\T_h$. Depth of the genesis block is defined as depth $0$. Afterwards, depth of each honest block $h_i$ is set equal to $1$ plus the depth of the last block that arrived before time $\tau^h_i$. Then, $d^h_i = i$ for any i. Finally, let $D_h(t)$ denote the depth of the last block that was mined before time $t$. Notice that $D_h(t)$ is a monotonically increasing process, and, at any given time $D_h(t)$ can increase by at most $1$. This implies that by time $t$, each depth from $1$ to $D_h(t)$ contains at least one honest block. Moreover, since $d^h_i = i$ for any i, $D_h(t)$ is equal to the number of honest blocks that were mined until time $t$. Since each honest block has a well defined depth in $\T_h$ and since each adversarial tree is rooted at some honest block; $\T_h$, in fact, acts as a common reference point for determining the depths of all the blocks in the system, including the adversarial blocks. 
Finally, let us define the following events which will be helpful for demonstrating the convergence of the longest chain in the subsequent sections:

$E_{ij}$ is the event that $D_i(t) < D_h(t-\Delta) - D_h(\tau^h_i)$ for all $t > \tau^h_j+\Delta$.
\begin{equation}
    F_j = \bigcap_{0 \leq i < j} E_{ij},
\end{equation}
$F_j$ is called the `adversary-proof' convergence event. 

These event defined above can be interpreted as about a fictitious system where there is a growing chain consisting of only honest blocks. The event $E_{ij}$ is the event that the adversarial tree rooted at the $i$-th honest block does not catch up with that honest chain any time after the generation of the $j$-th honest block. Such a tree can be interpreted as providing the resources for a possible attack at the honest chain. If $E_{ij}$ occurs, then there is not enough resource for the $i$-th tree to attack after the $j$-th block. If $F_j$ occurs, there is not enough resource for {\em any} of the previous trees to attack the honest chain. 

Even though the events are about a fictitious system with a purely honest chain and the longest chain in the actual system may consist of a mixture of adversarial and honest blocks, intuitively the actual chain can only grow faster than the fictitious honest chain, and so we have the following key lemmas \ref{lem:regen} and \ref{lem:loner}. These lemmas justify us giving the name {\em adversary-proof convergence event} to the event $F_j$.

For the proof of these lemmas, it is crucial to show that $D_h(t)$ gives a conservative bound on the growth of the chain $\C$ from time $s$ to $t$. For this purpose, before moving onto the lemmas \ref{lem:regen} and \ref{lem:loner}, we assert the following proposition:

\begin{proposition}
\label{prop:delay-0}
For any given $s$, $t$ such that $s < t$;
$$D_h(t) - D_h(s) \leq L(t)-L(s)$$
\end{proposition}

Proof follows from the fact that $D_h(s)-D_h(t)$ is equal to the number of honest blocks that were mined in the time interval $[s,t]$. Since each honest block is attached to the tip of $\C$ when it is mined, $L(t)-L(s)$ should be equal to, at least, the number of honest blocks mined in the interval $[s,t]$. Hence,
$$D_h(t) - D_h(s) \leq L(t)-L(s)$$

\begin{lemma}
\label{lem:regen}
When $\Delta=0$, if $F_j$ occurs, then the chain $\C(\tau^h_j)$ is a prefix of any future chain $\C(t)$, $t > \tau^h_j$. Equivalently, the $j$-th honest block will be in $\C(t)$ for all $t > \tau^h_j$. 
\end{lemma}

\begin{proof}
We will argue by contradiction. Suppose $F_j$ occurs and let $t^* > \tau^h_j$ be the smallest time such that $\C(\tau^h_j)$ is not a prefix of $\C(t)$. Let $h_i$ be the last honest block on $\C(t^*)$, which must exist as the genesis block is by definition honest. If $h_i$ is generated at some time $\tau^h_i> \tau^h_j$, then $\C(\tau^{h-}_i)$ is the prefix of $\C(t^*)$ before block $h_i$, and does not contain $\C(\tau^h_j)$ as a prefix, contradicting the minimality of $t^*$. So $h_i$ must be generated before $\tau^h_j$, implying that $i < j$. Then, the part of $\C(t^*)$ after block $h_i$ must lie entirely in the tree $\T_i(t^*-\tau^h_i)$ rooted at $h_i$. Hence, 
\begin{equation}
    L(t^*) \leq L(\tau^h_i) + D_i(t^*)
\end{equation}
However, we know that;
\begin{equation}
    D_i(t^*) < D_h(t^*)-D_h(\tau^h_i) \leq L(t^*)-L(\tau^h_i)
\end{equation}
where the first inequality follows from the fact that $F_j$ holds and the second inequality follows from proposition \ref{prop:delay-0}. From this we obtain that 
\begin{equation}
    L(\tau^h_i) + D_i(t^*) < L(t^*)
\end{equation}
which is a contradiction since $L(t^*) \leq L(\tau^h_i) + D_i(t^*)$. This concludes the proof.

\end{proof}
\end{comment}

In this section, we show that the adversary-proof convergence event occurs infinitely often if $\lambda_a < \lambda_h$, and will also give an estimate on how frequently that happens. This will imply persistence and liveness of the protocol with high probability guarantees.

\begin{lemma}
\label{lem:infinite_many_F_delta_0}
If 
$$\lambda_a < \lambda_h,$$
then there exists a constant $c>0$ such that $P(F_j) \geq c$ for all $j$. Then, with probability $1$, the event $F_j$ occurs for infinitely many $j$'s.
\end{lemma}

\begin{proof}

First, fix some large number $B$, and, let $B_1$ be the event that there exists an adversarial tree $\tt_i$ with depth equal to $A_h$ at some time $t$ such that $A_h(t)<j+B$. Similarly, let $B_2$ be the event that there exists an adversarial tree $\tt_i$ with depth equal to $A_h$ at some time $t$ such that $A_h(t) \geq j+B$. Now, we can express $P(F^c_j)$ in the following way:
$$P(F^c_j) = P(B_1) + P(B_2|B_1) (1-P(B_1))$$

Let $G_d$ be the event that the first block at depth $d$ is an honest block. Since $\lambda_h>\lambda_a$, ratio of the number of depths containing adversarial blocks over those containing honest blocks decays to zero as time increases. Consequently, $G_d$ happens infinitely often. Let $d'$ be the largest depth smaller than $j$ such that $G_{d'}$ happened. Then, with non-zero probability, the adversary has not mined any adversarial blocks from time $\tau^h_{d'}$ to the time $\tau^h_{j+B}$. This implies that $P(B_1)\leq c_0<1$ for some constant $c_0$. Moreover, $P(B_2|B_1)$ decays to $0$ as $B$ increases since the difference between the number of adversarial blocks and honest blocks mined after any fixed time drifts to $-\infty$. Consequently, for any large constant $B$, there exists a number $c_1<1$ such that $P(B_2|B_1)\leq c_1<1$. Then, 
$$P(F^c_j) \leq c_0 + c_1 (1-c_0) = c < 1$$
This completes the proof.

\end{proof} 

We next obtain a bound on the probability that, for blocks $j$ to $j+k-1$, there are no adversary-proof convergence events, i.e. a bound on:
$$P(\bigcap_{m \in \{j,..,j+k-1\}} F_m^c)$$

\begin{lemma}
\label{lem:pow-decay-delta-zero}
When $\Delta=0$,
$$P(\bigcap_{m=j,..,j+k-1} F^c_m) \leq A_1 e^{-A_2 k}$$ where $A_1$ is a constant, and, 
$$A_2 = -\ln(\frac{4\lambda_a\lambda_h}{(\lambda_a+\lambda_h)^2})$$.
\end{lemma}

\begin{proof}

First, observe that $F^c_m$, which we refer to as the `catch-up event', implies the existence of a minimum `catch-up' time $t_m \geq \tau^h_m$ such that there exists an adversarial tree $\tt_i$ extending from some honest block $h_i$, $i<m$, for which, the following holds: $$D_i(t_m) \geq A_h(t_m) - A_h(\tau^h_i).$$ 
Let $l_m := i$ denote the index $i$ of this tree. Although there can be multiple adversarial trees $\tt_i$ with different catch-up times $t \geq \tau^h_m$ such that $D_i(t) \geq A_h(t)-A_h(\tau^h_i)$, we only focus on the tree $\tt_{l_m}$ for which the catch-up time $t$ is the minimum among all others. In this context, let $r_m$ be the index of the last honest block before time $t_m$, $r_m := A_h(t_m)$. Since $t_m \geq \tau^h_m$ and $A_h$ is monotonically increasing, $r_m = A_h(t_m) \geq A_h(\tau^h_m) = m$. Combining this fact with our knowledge that $l_m < m$, we infer that $l_m < m \leq r_m$. (Refer to figure \ref{fig:catch-up} for an example diagram of the catch-up by tree $\tt_m$.)

\begin{figure}[hbp]
    \centering
    \includegraphics[width=\linewidth]{figures/sample-catch-up.jpg}
    \caption{Sample catch up event by the adversarial tree $\tt_{l_m}$.}
    \label{fig:catch-up}
\end{figure}

Now, at time $t_m$, there exists at least one adversary block from the tree $\tt_{l_m}$ at every depth from $l_m+1 \leq m$ to $r_m \geq m$. Hence, at time $t_m$, there are at least $r_m-l_m$ adversary blocks from depth $l_m+1$ to $r_m$. 

Notice that if $\bigcap_{m=j,..,j+k-1} F^c_m$ happens, then, there exists such adversarial trees $\tt_{l_m}$ and depths $l_m$ and $r_m$ as described above for every $m$, $j \leq m \leq j+k-1$. Let $l^*$ and $r^*$ denote the minimum and maximum values of $l_m$ and $r_m$ for $m=j,..,j+k-1$. Similarly, let $t^*$ denote the maximum of the associated catch-up times $t_m$. We observe since $H$ grows monotonically, the last catch-up event at time $t^*$ happens at depth $r^*$. Since $r_m \geq m$ and $l_m < m$ for all $m$, $l^*+1 \leq j$ to $r^* \geq j+k-1$. Then, we know from our observation above that, at time $t^*$, there exists at least one adversary block at every depth from $l^*+1 \leq j$ to $r^* \geq j+k-1$. Moreover, there is exactly $1$ honest block at each depth from $l^*+1$ to $r^*$. Consequently, if $\bigcap_{m=j,..,j+k-1} F^c_m$ happens, at least $1$ adversary blocks should have have been mined at every depth from $l^*+1$ to $r^*$ after time $\tau^h_{l^*}$ until time $t^*$ where $\tau^h_{r^*} \leq t^* < \tau^h_{r^*+1}$. (Refer to figure \ref{fig:interval} for an example diagram of the union of the intervals $[l_m,r_m]$.) Denoting this event by $G$, we conclude that $\bigcap_{m=j,..,j+k-1} F^c_m$ implies $G$:
$$\bigcap_{m=j,..,j+k-1} F^c_m \subseteq G$$

\begin{figure}[hbp]
    \centering
    \includegraphics[width=\linewidth]{figures/sample-interval.jpg}
    \caption{Union of the catch-up intervals for different adversarial trees. Note that there is at least one adversary block at each depth in the union of the intervals. Black circles denote the first and the last adversarial blocks in the adversarial trees. White and orange circles represent the honest blocks such that those denoted as orange are under attack by the adversary. Depths of these blocks are shown at the top. In this example, $l^*=l_j$, $r^*=r_{j+2}$, which implies $t_{j+2}=t^*$.}
    \label{fig:interval}
\end{figure}

Finally, we calculate an upper bound on the probability of $G$:
$$G \subseteq \bigcup_{0 \leq a < j,\ b \geq j+k-1} G_{a,b}$$
where $a$ and $b$ are fixed numbers, and, $G_{a,b}$ is the event that at least $1$ adversary block has been mined at each depth from $a$ to $b$ after time $\tau^h_a$ until time $\tau^{h-}_{b+1}$. In other words, $G_{a,b}$ is the event that at least $b-a$ adversary arrival events have occurred after time $\tau^h_a$ until time $\tau^{h-}_{b+1}$. Let $\tau^a_i$ be the mining time of the $i$-th adversary block mined after time $\tau^h_a$ for $i = 1,2,\cdots,b-a$. 
And define $\delta^h_i = \tau^h_{a+i} - \tau^h_{a+i-1}$ and $\delta^a_i = \tau^a_i - \tau^a_{i-1}$ $i = 1,2,\cdots,b-a$ as the inter-arrival times for honest and adversary blocks respectively ($\tau^a_0 := \tau^h_a$).
Then, the probability of $G_{a,b}$ becomes;
$$P(G_{a,b}) = P(\{\sum_{i=1}^{b-a+1} \delta^h_i > \sum_{i=1}^{b-a} \delta^a_i\}).$$
Next, defining $T_i := \delta^h_i-\delta^a_i$, we observe that;
\begin{IEEEeqnarray*}{rCl}
P(\sum_{i=1}^{b-a+1} \delta^h_i > \sum_{i=1}^{b-a} \delta^a_i) &=& P(\delta^h_{b+a+1} + \sum_{i=1}^{b-a} (\delta^h_i-\delta^a_i) > 0) \\
&=& P(\delta^h_{b+a+1} + \sum_{i=1}^{b-a} T_i > 0). 
\end{IEEEeqnarray*}
Then, we obtain a Chernoff bound for $P(G_{a,b})$ with parameter $s>0$:
\begin{IEEEeqnarray*}{rCl}
P(G_{a,b}) &=& P(\delta^h_{b+a+1} + \sum_{i=1}^{b-a} T_i > 0) \\
&\leq& E[e^{s\delta^h_{b+a+1}}e^{s\sum_{i=1}^{b-a} T_i}] \\
&=& E[e^{s\delta^h_{b+a+1}}\prod_{i=1}^{b-a} e^{s T_i}] \\
&=& E[e^{s\delta^h_{b+a+1}}] \prod_{i=1}^{b-a} E[e^{s T_1}] \\
\end{IEEEeqnarray*}
where we can take the product out of the expectation as $T_i$ are i.i.d random variables. Here, minimizing $E[e^{s T_1}]$ with respect to $s$ for the exponentially distributed $\delta^h_1$ and $\delta^a_1$ with parameters $\lambda_h$ and $\lambda_a$, $\lambda_h > \lambda_a$, yields
$$P(G_{a,b}) \leq 2(\frac{4\lambda_h\lambda_a}{(\lambda_a+\lambda_h)^2})^{a-b} < 1$$
Then, using the union bound, we can state that;
\begin{IEEEeqnarray*}{rCl}
P(\bigcap_{m=j,..,j+k-1} F^c_m) &\leq& P(G) \\
&\leq& \sum_{0 \leq a<j} \sum_{b \geq j+k-1} P(G_{a,b}) \\
&\leq& 2\sum_{0 \leq a<j} \sum_{b \geq j+k-1} (\frac{4\lambda_h\lambda_a}{(\lambda_a+\lambda_h)^2})^{b-a} \\
&\leq& 2(\frac{4\lambda_h\lambda_a}{(\lambda_a+\lambda_h)^2})^{k} \sum_{a=0}^{\infty} \sum_{b=0}^{\infty} (\frac{4\lambda_h\lambda_a}{(\lambda_a+\lambda_h)^2})^{a+b} \\
&\leq& A_1 (\frac{4\lambda_h\lambda_a}{(\lambda_a+\lambda_h)^2})^{k} \\
\end{IEEEeqnarray*}
for $\Delta=0$. Here, 
$$A_1 = 2(\frac{1}{1-e^{-A_2}})^2,$$
and, $A_2$ is as defined in the proposition. This concludes the proof.

\end{proof}

If $\lambda_a > \lambda_h$, we know that the adversary can always attack the honest chain by growing a side chain at a rate faster than the honest chain's growth rate and replace it at will. However, the adversary-proof convergence event $F_j$ has a non-zero probability of occurrence if $\lambda_a < \lambda_h$, and, this implies that no attack works since the event $F_j$ occurs for infinitely many $j$'s. This shows the tightness of the threshold $\beta = 1/2$ when $\Delta=0$. 
